YODA: Teacher-Student Progressive Learning for Language Models

Although large language models (LLMs) have demonstrated adeptness in a range of tasks, they still lag behind human learning efficiency. This disparity is often linked to the inherent human capacity to learn from basic examples, gradually generalize and handle more complex problems, and refine their skills with continuous feedback. Inspired by this, this paper introduces YODA, a novel teacher-student progressive learning framework that emulates the teacher-student education process to improve the efficacy of model fine-tuning. The framework operates on an interactive \textit{basic-generalized-harder} loop. The teacher agent provides tailored feedback on the student's answers, and systematically organizes the education process. This process unfolds by teaching the student basic examples, reinforcing understanding through generalized questions, and then enhancing learning by posing questions with progressively enhanced complexity. With the teacher's guidance, the student learns to iteratively refine its answer with feedback, and forms a robust and comprehensive understanding of the posed questions. The systematic procedural data, which reflects the progressive learning process of humans, is then utilized for model training. Taking math reasoning as a testbed, experiments show that training LLaMA2 with data from YODA improves SFT with significant performance gain (+17.01\% on GSM8K and +9.98\% on MATH). In addition, we find that training with curriculum learning further improves learning robustness.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

The rapid advancements in Large Language Models (LLMs) have significantly transformed the fields of natural language processing and artificial intelligence. These models demonstrate remarkable proficiency across a spectrum of general tasks, ranging from writing  to code synthesis. 
Despite its general capability, their reasoning capability is still in its infancy compared to advanced human reasoning capability and learning efficiency.
\input{figures/motivation}
In contrast to machines, which depend on extensive datasets for learning and problem-solving, humans possess the unique ability to master diverse skills through a limited number of examples. This remarkable human capacity inspires a rethinking of model learning strategies, particularly highlighting the 'fundamental-similar-harder' cycle in human education. 
In this approach, teachers initially focus on foundational problem-solving techniques. Students then consolidate their understanding by applying these principles to similar problems, and eventually, they tackle increasingly complex challenges, thus enhancing their problem-solving skills.
Crucially, this educational journey is marked by continuous guidance and feedback from teachers. Students learn to identify and correct their mistakes, refining their approach for more reliable problem-solving. 
This approach highlights the possibility of rethinking the training methodologies for LLMs. Rather than solely depending on vast datasets, could we devise a learning methodology for LLMs that mirrors the nuanced and adaptive learning processes of humans?"


% Unlike machines, which rely on vast datasets for learning task-solving, humans adeptly learn to master various skills from limited examples. 
% Drawing inspiration from the effective learning strategies in human education, a stands-out learning circle is ``\textit{fundamental-similar-harder}'' process: teacher encourages students to learn fundamental question-solving, then master similar question types by extrapolating from learned examples, and progressively strengthen problem-solving skills by learning complex challenges. 
% to comprehend and master similar question types by extrapolating from limited examples, and progressively improve problem-solving skills by methodically progressing to solving more complex challenges.  
% Crucially, throughout this teacher-guided journey, students continually learn from their mistakes pointed out by the teacher and make self-refinement, ensuring a more dependable problem-solving process.
% Recognizing the benefits of human learning methods, there's a clear need for a new approach to LLM training. Instead of just relying on large amounts of data, what if we could train models in a way more like how humans learn?
To advance model learning inspired by human educational strategies, we present \method, a novel multi-agent interactive learning framework. This framework mimics the interactive dynamics of a traditional educational setting and comprises two distinct agents: the 'student' agent, tasked with providing and refining answers, and the 'teacher' agent, responsible for guiding the learning process.
The student agent endeavors to respond to questions, refining its answers based on the feedback received. 
In contrast, the teacher agent offers crucial feedback and introduces new questions. 
These questions are systematically structured to reinforce the student's understanding through similar questions, and to incrementally enhance its problem-solving skills with more complex questions.
The interaction between these agents follows a progressive 'fundamental-similar-harder' loop. Initially, the student agent focuses on basic problem-solving, refining its responses until they meet the teacher's evaluation standard. Subsequently, to solidify the student's understanding, the teacher poses conceptually similar questions. Once the student demonstrates mastery over fundamental problems, the teacher raises the difficulty by introducing more complex challenges.
This systematic progression not only cultivates the student's problem-solving abilities but also bolsters learning robustness through an iterative process of feedback and refinement. 
Finally, the procedural data automatically synthesized in the learning loop are applied for model tuning, which reduces data scarcity problem by only requiring unlabelled fundamental questions as the starting points.
% To promote model learning with a human-learning strategy, we propose a novel multi-agent interactive learning framework to stimulate of this approach, which 
% interplays a student agent who wants to learn, and a teacher agent that guides the learning process.
% The student model tries to answer questions and refine answers with teacher evaluation, and the teacher agent is responsible for giving feedback and posing new, generalized similar questions or harder complex questions.
% Specifically, they interact in a progressive loop: ``{fundamental-similar-harder}''. 
% To begin with, the student learns fundamental problem-solving by iteratively refining its answer until it's judged as correct by the teacher. 
% To further help the student to consolidate its understanding by learning from similar question types, the teacher agent poses conceptually similar questions for testing. 
% Afterward, if the student can completely master the questions with fundamental difficulty, the teacher progressively enhances student learning by testing it with more complex problems. 
% Overall, this progressive learning process forms students' problem-solving ability in a systematic manner. 
% It further enhances learning robustness by iterative feedback-refinement interaction.
% Finally, the data automatically synthesized in the learning process are applied for model tuning, which reduces data scarcity problem by only requiring unlabelled fundamental questions as the starting points.
% It is worth noting that the student and teacher can be different agents role-played by the same model, to enhance the flexibility of the whole process. 
\input{figures/multi-agent-figure-original}

Experimental results show that the LLaMA2~\citep{llama2} model trained with automatic procedural data, significantly outperforms both baseline models and those trained with human supervision in mathematical benchmarks. This success highlights the effectiveness of a progressive learning strategy, mirroring human education, in enhancing model capabilities. Our in-depth analysis reveals that exposing the model to a sequence of increasingly complex questions solidifies its knowledge and sharpens its reasoning. An iterative feedback-refinement cycle also played a crucial role in strengthening the learning process. Additionally, integrating computational tools in the latter stages of problem-solving further improved performance by 20\%.

% Experimental results demonstrate that training a less advanced model, LLaMa2, with procedural data derived from GPT-4 leads to significant improvements in mathematical benchmarks, surpassing both baseline models and human-supervised counterparts, which shows the efficacy of promotes model learning by progressive learning strategy of humans. 
% A deeper analysis underscores the efficacy of our approach, highlighting that exposure to similar and progressively complex questions enables the model to solidify its knowledge and enhance reasoning capabilities. The iterative feedback-refinement process further enhances learning robustness.
% Further using calculation tools to enhance the final-step calculation can additionally promote performance by 20\% points. 
The key contributions can be summarized as follows:
(1) We developed a progressive multi-agent cooperative learning framework. It enhances model learning through a systematic 'fundamental-similar-harder' approach and improves robustness with an iterative 'feedback-refinement' strategy.
(2) Our methodology addresses data scarcity by incrementally expanding the data scope, beginning with a small set of unlabeled problems and progressively widening.
(3) Experiments show that our approach significantly outperforms baseline models and those trained under human supervision, demonstrating marked improvements in performance.


% \input{tables/comparative}


==> tables/comparative.tex <==
\begin{table}[h]
\centering
\caption{\label{tab:effect-teacher-student-loop}Comparative Analysis of Accuracy with and without Teacher-Student Loop.
We compare the results of using a single student model (Zero-shot COT) against the teacher-feedback-student-revision approach. 
The results are conducted on a sample of 1000 training prompts from both the GSM8K and Math datasets. }
\label{tab:teacher-student-loop}
\begin{tabular}{lll}
\toprule
Model &  GSM8K &  Math \\
\midrule
\midrule
Student & 81.8\% & 35.1\% \\
Teacher-Student Loop & 85.1\% & 36.4\% \\
\bottomrule
\end{tabular}
\end{table}

==> tables/data_size_effect.tex <==
\begin{table}[h]\scriptsize
    \centering
    \caption{\label{tab:data-size-effect}
    % A "-" symbol indicates the absence of results for certain cases.
    }
     \scalebox{1.5}{
    \begin{tabular}{l|cc}
    \toprule
    Models&\textbf{GSM8K}&\textbf{MATH}\\
    \midrule
    \midrule
    
     \bottomrule
    \end{tabular}
    }
\end{table}


==> tables/filtering.tex <==
\begin{table}[!ht]\scriptsize
    \centering
    \caption{Performance comparison of our approach with and without ground truth filtering on the GSM8K and Math datasets.}
    \begin{tabular}{l|cc}
    \toprule
    Models & \textbf{GSM8K} & \textbf{MATH}   \\
    \midrule
    \midrule
   YODA & 52.84 & 13.74  \\
   YODA + GT-filter & 53.60 & 14.56  \\
    \bottomrule
    \end{tabular}
    \label{tab:performance-with-without-filtering}
\end{table}
